VIA: Analyzing Device Interfaces of Protected Virtual Machines

Both AMD and Intel have presented technologies for confidential computing in cloud environments. The proposed solutions - AMD SEV (-ES, -SNP) and Intel TDX - protect Virtual Machines (VMs) against attacks from higher privileged layers through memory encryption and integrity protection. This model of computation draws a new trust boundary between virtual devices and the VM, which in so far lacks thorough examination. In this paper, we therefore present an analysis of the virtual device interface and discuss several attack vectors against a protected VM. Further, we develop and evaluate VIA, an automated analysis tool to detect cases of improper sanitization of input recieved via the virtual device interface. VIA improves upon existing approaches for the automated analysis of device interfaces in the following aspects: (i) support for virtualization relevant buses, (ii) efficient Direct Memory Access (DMA) support and (iii) performance. VIA builds upon the Linux Kernel Library and clang's libfuzzer to fuzz the communication between the driver and the device via MMIO, PIO, and DMA. An evaluation of VIA shows that it performs 570 executions per second on average and improves performance compared to existing approaches by an average factor of 2706. Using VIA, we analyzed 22 drivers in Linux 5.10.0-rc6, thereby uncovering 50 bugs and initiating multiple patches to the virtual device driver interface of Linux. To prove our findings criticality under the threat model of AMD SEV and Intel TDX, we showcase three exemplary attacks based on the bugs found. The attacks enable a malicious hypervisor to corrupt the memory and gain code execution in protected VMs with SEV-ES and are theoretically applicable to SEV-SNP and TDX.

==> evaluation_hc.tex <==
\section{Evaluation}\label{sec:eval}
In this section, we first categorize the bugs uncovered in the virtual device interface
and present three exploits based on the discovered bugs.
Finally, we evaluate the performance of \coolname{}.

\subsection{Bug Overview}
\begin{table}
	\caption{List of examined drivers with their type,
	communication interface and number of discovered bugs.
	\textit{QVD} stands for QEMU Virtual Device,
	and \textit{CVM} for Google Confidential \gls{VM}.
	We distinguish between low and high severity bugs.
	An analysis of each bug can be found in our repository~\cite{fuzzsarepo}.}

\begin{center}
\begin{threeparttable}%
\begin{tabular}{ l c c c c c }
 \toprule
	\multirow{2}{*}{Driver} & \multirow{2}{*}{Usage} & \multirow{2}{*}{Type} & \multirow{2}{*}{Bus} & \multicolumn{2}{c}{\#Bugs} \\
			     &                     &                    &                   & Low & High \\
 \midrule
	virtio\_ring & QVD & Common & VIO & 2 & 4 \\
	virtio\_net & QVD & NET & VIO & 1 & 1 \\
	virtio\_blk & QVD & BLK & VIO & 5 & 1 \\
	virtio\_crypto & QVD & CRYPTO & VIO & 2 & 0 \\
	virtio\_rng & QVD & RNG & VIO & 0 & 1 \\
	virtio\_console & QVD & MISC & VIO & 1 & 0 \\
	virtio\_balloon & QVD & MISC & VIO & 2 & 1 \\
	\rowcolor{lightgray} virtio\_input & QVD & MISC & VIO & 0 & 0 \\
	rocker & QVD & NET & PCI & 1 & 3 \\
	sungem & QVD & NET & PCI & 1 & 0\textsuperscript{*} \\
	sunhme & QVD & NET & PCI & 2 & 0\textsuperscript{*} \\
	8139cp & QVD & NET & PCI & 1 & 0 \\
	vmxnet3 & QVD & NET & PCI & 0 & 5 \\
	\rowcolor{lightgray} ne2k-pci & QVD & NET & PCI & 0 & 0 \\
	e100 & QVD & NET & PCI & 0 & 1 \\
	e1000 & QVD & NET & PCI & 0 & 3 \\
	e1000e & QVD & NET & PCI & 1 & 0 \\
	qemu\_fw\_cfg & QVD & MISC & PLT & 1 & 0 \\
	acpi & QVD & MISC & PLT & 0 & 1 \\
	gve & CVM & NET & PCI & 2 & 3 \\
	nvme & CVM & BLK & PCI & 1 & 1 \\
	tpm\_tis & CVM & TPM & PLT & 0 & 2 \\
 \bottomrule
\end{tabular}
\end{threeparttable}%
\end{center}
  \begin{tablenotes}[flushleft]
    \item \scriptsize{\textsuperscript{*} Device-controlled values passed to \texttt{swiotlb\_tbl\_unmap\_single} as described in
Section 6.2 were not counted as separate bugs.}
  \end{tablenotes}
\label{tbl:all_bugs}
\end{table}
\coolname{} was used to examine a total of \drvanalyzed drivers in the Linux kernel with version \kernelversion.
Of the analyzed drivers, \drvanalyzedqvd belong to QEMU virtual devices and \drvanalyzedcvm to specialized hardware available in Google's SEV-enabled confidential computing VM~\cite{googlecvm}.
The analysis was performed via intermittent runs over the course of several months (i.e., from November 2020 to February 2021). %
Each fuzzing session usually lasted between a few minutes to several hours.
We responsibly disclosed found security issues with the respective maintainers.
To prepare the drivers for the dynamic analysis, we patched problematic code where possible by adding proper sanitization.
Additionally, we removed complex checks (e.g., checksum comparisons) on data provided by the fuzzer.
This optimization was applied to the drivers \texttt{e1000}, \texttt{rocker} and \texttt{sungem}.
Addressing such issues in a generic way is an orthogonal problem that has been addressed in other works~\cite{Aschermann2019,Chen2019}.
The required modifications were easy to identify from the kernel or crash log, and workarounds could easily be developed.
We list the changes to the driver code in our public repository~\cite{fuzzsarepo}.

In total, \coolname{} uncovered \nbugs novel bugs across the drivers listed in Table~\ref{tbl:all_bugs}.
At the time of writing, \nbugsconf of the discovered bugs in
\texttt{swiotlb},
\texttt{gve},
\texttt{virtio\_ring},
\texttt{virtio\_net} and
\texttt{vmxnet3}
have been, or are currently being fixed~\cite{vmxnet3,virtionet0,swiotlb0,virtioring1,virtioring2,virtioring0,virtioring3,virtioring4,gve0,gve1}.
Each entry was carefully validated by examining the source code of the offending driver, and bug duplicates were removed.
A thorough analysis of each bug is available in our repository~\cite{fuzzsarepo}.
The types of bugs covered include out-of-bounds access, device-shared pointer, invalid memory access, slab management bugs, miscellaneous bugs, assertion failure, unbound memory allocations, and deadlocks.
We distinguish between bugs of high and low severity.
We consider bugs as severe that potentially leak or corrupt guest memory either on their own or by aiding exploitation of different vulnerabilities.
These include out-of-bounds access, device-shared pointer and slab management bugs, such as use-after-free or double-free.
The remaining bug classes are considered low-severity, as they will impact the guest system's availability but likely do not undermine the security guarantees of \gls{SEV} or \gls{TDX}.
Low-severity bugs usually arise from implementation errors, that should be fixed to guarantee proper functionality of the driver.

\begin{table}
\caption{
  Distribution of bug classes found by \coolname{}.
}
\begin{center}
\begin{tabular}{ l c }
 \toprule
 Bug Class & Count \\
 \midrule
 Out-of-Bounds access & 14 \\
 Invalid memory access & 10 \\
 Slab management & 8 \\
 Device-shared pointer & 5 \\
 Miscellaneous & 3 \\ %
 Assertion failure (\texttt{BUG}) & 4 \\
 Unbounded allocation & 5 \\
 Deadlock & 1 \\
 \bottomrule
\end{tabular}
\end{center}
\label{tbl:fuzz_bugs}
\end{table}


Table~\ref{tbl:fuzz_bugs} lists the bug classes and the corresponding number of discovered bugs.
Among the most common bugs are \textit{Out-of-Bounds access} and \textit{Invalid memory access} bugs, with respectively $14$ and $10$ incidents.
The discovered root cause of these two classes is missing validation for the index and length fields of shared data structures.
Next are \textit{slab management} bugs encompassing $8$ instances of use-after-free or double free issues.
Such bugs often occur in the teardown code of a function if error handling is incorrectly implemented.
Further, \coolname{} uncovered $5$ \textit{device-shared pointer} bugs where a \gls{VM} kernel pointer is stored in shared memory. %
These device-shared pointer issues were all present in few network drivers (\texttt{GVE}, \texttt{e100}, \texttt{rocker}, \texttt{vmxnet3}).
The \textit{miscellaneous} bug category comprises of $3$ unique bugs including missing synchronization of device memory, division by zero and limited directory traversal.
Lastly, our fuzzing setup caught $4$ cases of assertions failures, $5$ unbounded memory allocations and $1$ deadlock.
The \textit{assertion failure} class includes cases when the kernel would detect an unexpected state and call \texttt{BUG()}.
The \textit{unbound memory allocations} category considers cases for which the kernel performs large allocations or fails to free allocated memory, leading to out-of-memory conditions.
\textit{Deadlocks} can occur, if data from the device introduces a \gls{VM} state in which a kernel thread is indefinitely waiting for a resource.




\subsection{A Case Study of Three Bugs}\label{sec:case-study}

In this section we discuss how a malicious administrator, with only access to the QEMU process, can exploit
three of the discovered bugs to overwrite secret memory of a virtual machine and to gain code execution inside the virtual machine.

The exploitation of the three bugs was performed on a virtual machine protected with \gls{SEV-ES} and running Linux \kernelversionbugs. %
The exploits were designed with \gls{KASLR} disabled, though a malicious \gls{HV} can use leaked \gls{VM} kernel pointers to
infer the memory layout of the \gls{VM} if required.



\paragraph{Device-shared pointer in vmxnet3}
\begin{figure}[htbp]
    \begin{lstlisting}[style=CStyle, escapechar=!]
struct vmxnet3_rx_buf_info {
	struct sk_buff *skb; // shared ptr with device
	...
};
struct sk_buff {
	void (*destructor)(struct sk_buff *skb);
	...
};
void skb_release_head_state(struct sk_buff *skb) {
	if (skb->destructor) skb->destructor(skb);
}\end{lstlisting}
	\caption{Vulnerable code in the \texttt{vmxnet3} driver. %
	The pointer \texttt{skb} on Line 2 is accessible by the device and can be overwritten.
	By creating a fake \texttt{skb} object and overwriting the pointer, the device can trick the driver into calling any function on Line 12.}
\label{code:vmxnet3_desc}
\end{figure}


The \texttt{vmxnet3} interface relies on an array of descriptors that can be accessed by the device.
A \texttt{vmxnet3} descriptor, shown in Figure~\ref{code:vmxnet3_desc}, contains an associated \texttt{skb} kernel pointer among other fields.
The pointer points to a pre-allocated \texttt{sk\_buff} object in the \gls{VM}'s private memory, which can be used immediately when a network packet is received.

The exposure of this pointer to an untrusted device leaks information about the VM kernel's randomized address space and additionally allows a malicious \gls{HV} to overwrite the pointer with a convenient value.
When the packet is received, the contents of the \texttt{sk\_buff} are parsed, and the object is eventually freed.
Before freeing the packet, the \texttt{sk\_buff}'s destructor would be called, as shown on Line 12.

 In order to exploit the bug the \gls{HV}
overwrites the \texttt{skb} pointer in the descriptor to point to decrypted memory at the moment of sending a packet to the \gls{VM}.
At the same time, the \gls{HV} forges a fake \texttt{sk\_buff} object at the new address and overwrites the destructor pointer to a suitable code gadget in the \gls{VM}'s kernel.
The code gadget would position the stack into decrypted memory, which would then allow continuing execution using return-oriented programming.
We determined empirically that many code gadgets are suitable destructor pointers because many registers and the stack contain the address of the \texttt{skb} in decrypted memory.
Similar exploitation opportunities were found in the driver implementations of \texttt{GVE}, \texttt{e100}, and \texttt{Rocker}.




\paragraph{Use-after-Free bug in \gls{VIRTIO}-Net}
\begin{figure}[htbp]
  \begin{lstlisting}[style=CStyle]
static int virtnet_probe(struct virtio_device *vdev) {
  ...
  struct net_device *dev;
  struct virtnet_info *vi;
  ...
  dev = alloc_etherdev_mq(sizeof(struct virtnet_info), max_queue_pairs);
  ...
  vi = netdev_priv(dev); // vi lies within net_device memory area
  ...
  if (virtio_has_feature(vdev, VIRTIO_NET_F_MTU)) {
    mtu = virtio_cread16(vdev, offsetof(struct virtio_net_config, mtu));
    if (mtu < dev->min_mtu) { // check fails
      goto free;
  ...
free:
  free_netdev(dev); // struct net_device is freed
  return err;       // err == 0
}
static void virtnet_remove(struct virtio_device *vdev)
{
  struct virtnet_info *vi = vdev->priv;
  ...
  unregister_netdev(vi->dev); // vi->dev is device controlled
  ...
}
\end{lstlisting}
	\caption{
	  The \gls{HV} can induce \texttt{virtnet\_probe} to fail by providing a low \texttt{mtu} value.
	  The driver fails to set \texttt{err} correctly.
	  This leads to access of the freed memory, pointed to by \texttt{vi}, during device removal.}
\label{code:virtio_probe}
\end{figure}

\begin{figure}[htbp]
  \begin{lstlisting}[style=CStyle]
static void e1000_dump_eeprom(struct e1000_adapter *adapter) {
  ...
  eeprom.len = ops->get_eeprom_len(netdev); // HV controls eeprom.len
  ...
  data = kmalloc(eeprom.len, GFP_KERNEL); // data will overlap virtnet_info
  ...
  ops->get_eeprom(netdev, &eeprom, data); // HV controlled data is copied
  ...
  kfree(data);
}
\end{lstlisting}
	\caption{
	  The function \texttt{e1000\_dump\_eeprom} is used to gain control over the memory freed in \texttt{virtnet\_probe}.
	  The \gls{HV} controls \texttt{eeprom.len}.
	  The function \texttt{get\_eeprom} fills the allocated buffer with data controlled by the \gls{HV}.}
\label{code:e1000}
\end{figure}
The \texttt{virtio\_net} driver fails to return an error code if the initialization fails due to an invalid \texttt{mtu} value provided by the \gls{HV}.
This leads to a \textit{use-after-free} bug when the device is removed.
The vulnerable code is depicted in Figure~\ref{code:virtio_probe}.
To exploit this bug the \gls{HV} first attaches the \texttt{virtio\_net} device and causes \texttt{virtnet\_probe} to fail by providing a low \texttt{mtu} value.
To obtain control over the freed memory area, the \gls{HV} then attaches the \texttt{e1000} device
and triggers the code path shown in Figure~\ref{code:e1000}.
Specifying an \texttt{eeprom.len} of $0x1000$ will cause a new allocation in the \textit{kmalloc-4k} cache, which overlaps the memory area of the freed \texttt{struct virtnet\_info}.
The structure \texttt{virtnet\_info} contains the field \texttt{dev}, which points to a \texttt{net\_device} structure.
The \texttt{net\_device} structure contains the function pointer \texttt{ndo\_uninit}, that will be called in \texttt{unregister\_netdev} via the invocation of \texttt{virtnet\_remove}.
Similar to the previous exploit, the \gls{HV} overwrites \texttt{virtnet\_info->dev} to point to a decrypted memory area and sets \texttt{ndo\_uninit} to point to a suitable code gadget.
Next the \gls{HV} detaches the \texttt{virtio\_net} device to trigger the vulnerable code path and gain code execution.

The reliability of the exploit relies on two factors.
First, the allocation of the data allocated in \texttt{e1000\_dump\_eeprom} has to overlap the freed \texttt{struct net\_device}.
Second, the re-allocated memory area should not be overwritten before \texttt{virtnet\_remove} is called.
Under \gls{SEV}-(-ES, -SNP) the \gls{HV} has read access to encrypted memory.
This allows the \gls{HV} to infer the host virtual addresses of both allocations by monitoring changes to encrypted memory at suitable points during the interaction between the device and the driver\footnote{Alternatively, page fault side channels~\cite{li2019exploiting} could be used to infer address information.}.
In order to verify whether the data was overwritten,
the \gls{HV} compares the encrypted memory state after \texttt{e1000\_dump\_eeprom} to the current state before detaching the \texttt{virtio\_net} device.
If the inferred addresses differ or the memory has been overwritten
the \gls{HV} can either repeat the exploit attempt by
attaching a new device, or choose to abort the attempt.

\paragraph{Out-of-Bounds bug in \gls{VIRTIO} / swiotlb}
Every \gls{VIRTIO} driver in Linux relies on a common \gls{VIRTIO} interface implementation that handles the state of each communication queue.
Each queue is associated with an array of descriptors, depicted in Figure~\ref{code:virtio_desc}.
When a device sends a payload to the driver, the device typically only reads but does not update the \texttt{addr} and \texttt{len} fields since they are provided by the driver.

\begin{figure}[htbp]
    \begin{lstlisting}[style=CStyle]
struct vring_desc {
	__virtio64 addr;
	__virtio32 len; // not validated.
	__virtio16 flags;
	__virtio16 next;
};\end{lstlisting}
	\caption{
		Contents of a \gls{VIRTIO} descriptor. The device-controlled value of \texttt{len} is not validated and is used as an argument to \texttt{memcpy}.}
\label{code:virtio_desc}
\end{figure}

When a \gls{VM} uses AMD \gls{SEV} or Intel \gls{TDX}, the \gls{VIRTIO} implementation relies on the DMA API and its swiotlb implementation.
The swiotlb layer allocates a shared memory region used for communication.
A device copies a payload to this region, the swiotlb layer performs some validations and finally \textit{bounces} the payload to the driver's private buffer when memory is synchronized.
The length of the copied data is given by the \texttt{len} field of the \texttt{vring\_desc} structure, shown in Figure~\ref{code:virtio_desc}.

Our fuzzing tool uncovered that the swiotlb layer does not validate the device-controlled length of the memory copy, which causes a buffer overflow.
This allows a malicious device to overwrite the private memory of a protected \gls{VM} with arbitrary data of arbitrary length.
This vulnerability occurs in shared code by all Linux \gls{VIRTIO} drivers.
What area of private memory can be overwritten depends on the memory allocator used by the driver.
For example, \texttt{virtio\_console} and \texttt{virtio\_rng} would allow overflowing a buffer allocated from the Linux SLAB allocator.
We verified empirically that \texttt{net\_device} structures, e.g. allocated during the initialization of the \texttt{e1000} device,
are often allocated in proximity to the descriptor buffers allocated in \texttt{virtio\_console}.
In such cases the \gls{HV} can exploit the out-of-bounds bug to overwrite the contents of the structure and craft an exploit similar to the previous example.

To increase the reliability of the exploit, the \gls{HV} infers the host virtual addresses of the descriptor buffers as well as the \texttt{net\_device} structures
by observing changes in encrypted memory.
Based on the inferred addresses, the \gls{HV} selects a descriptor that points to a buffer that is allocated in proximity to one of the \texttt{net\_device} structures
and adjusts the descriptors \texttt{len} field to overwrite the \texttt{net\_device} memory area.
If no suitable locations are found the \gls{HV} re-attaches the devices until a suitable combination of descriptor buffer and \texttt{net\_device} addresses is detected.



\subsection{Performance Analysis}

In this section, we evaluate the performance of \coolname{}.
We compare \coolname{} against a state-of-the-art \gls{VM}-based approach.
Further, we examine whether \textit{delay reduction} and \textit{targeted interrupt injection} are effective in improving fuzzing performance.
We conducted all of our experiments on a machine equipped with an 8-Core Intel i7-7700 and 64GB of memory.
The analysis of each driver was restricted to one CPU core, to eliminate differences in performance due to the multithreaded design of \coolname{}.
In order to reduce randomness, we used an empty initial corpus and a fixed random seed for all evaluations.
The size of individual corpus files was limited to $10$kB and a timeout of 120 seconds per fuzzing iteration was used.
The harness modules used for the evaluation are listed in our public repository~\cite{fuzzsarepo}.

\begin{table}
  \caption{Comparison of executions per second and path coverage,
    between Agamotto~\cite{agamotto} and \coolname{} without (-D) and with (-ND) delay reduction,
    averaged over three hours.
    The evaluation was performed using the basic harness module, which performs one driver load/unload cycle.
    }
  \begin{center}
    \resizebox{\columnwidth}{!}{
    \begin{threeparttable}
      \begin{tabular}{l r r r @{}c r r}
	\toprule
	& \multicolumn{3}{c}{{\# Executions / s}}
	&
	& \multicolumn{2}{c}{{\# Paths}}
	\\
	\cmidrule{2-4}
	\cmidrule{6-7}
	& \thead{Agamotto} & \thead{\coolname-D} & \thead{\coolname-ND}
	&
	& \thead{Agamotto} & \thead{\coolname-ND}
	\\

	\midrule
	          8139cp & 1.39  &  1336.00 &  1275.50 & &  47 & 421 \\
                    e100 & 0.45  &    64.00 &   710.50 & & 303 & 442 \\
                   e1000 & 0.73  &     1.00 &    66.50 & &  40 & 829 \\
                  e1000e & 0.74  &    28.00 &   886.00 & &  60 & 890 \\
                     gve & 1.06  &     1.00 &   732.19 & &  32 & 148 \\
                ne2k-pci & 0.35  &  6604.00 &  6332.00 & &  27 &  21 \\
                    nvme & 0.79  &     0.02 &     1.55 & &  95 & 268 \\
                  rocker & 0.64  &  2752.00 &  4227.50 & &  35 &  54 \\
                  sungem & 0.98  &  3144.00 &  6199.50 & &  43 & 428 \\
                  sunhme & 1.14  &   786.00 &  1250.50 & &  40 & 440 \\
                 vmxnet3 & 0.74  &  2557.00 &  2735.00 & &  52 & 474 \\
	\bottomrule
      \end{tabular}
    \end{threeparttable}
  }
  \end{center}
\label{tbl:agamotto}
\end{table}


To evaluate the performance improvement compared to previous \gls{VM}-based approaches, we compare \coolname{}
against Agamotto~\cite{agamotto}, which is a state-of-the-art \gls{PCI} device fuzzer.
Agamotto is similar to USBFuzz~\cite{Peng2020} in function and performance.
It utilizes a virtual device which generates a mutated IO-stream that is
forwarded to the target driver. In addition, Agamotto uses dynamic checkpoints to speed up the analysis.
The evaluation was performed using a simple harness that loads and unloads a target driver, which is the only harness supported by Agamotto.
Targeted interrupt injection was enabled for each driver.
Each driver was analyzed for three hours and no modifications were applied to the driver code.
The results of the evaluation can be seen in Table~\ref{tbl:agamotto}.
On average \coolname{} improves the number of executed units per second by a factor of $1915$ and $2706$ for the delayed and non-delayed versions respectively.
In addition, \coolname{} improves average path coverage by a factor of $5.7$ by also mutating data read via the \gls{DMA} interface.
During the analysis \coolname{} repeatedly triggered two bugs in the \texttt{gve} and \texttt{nvme} drivers, while Agamotto triggered none.


\begin{table}
    \caption{
      Comparison of executions per second and path coverage without (-D) and with (-ND) delay reduction,
      averaged over three hours.
      The evaluation was performed using the extended harness modules, which interact with resources instantiated by the target drivers.
    }
  \begin{center}
    \begin{threeparttable}
      \begin{tabular}{l r r@{ }r @{}c r r}
	\toprule
	& \multicolumn{3}{c}{{\# Executions / s}}
	&
	& \multicolumn{2}{c}{{\# Paths}}
	\\
	\cmidrule{2-4}
	\cmidrule{6-7}
	& \thead{\coolname-D} & \multicolumn{2}{c}{\thead{\coolname-ND\\\bf{(Increase)}}}
	&
	& \thead{\coolname-D} & \thead{\coolname-ND}
	\\
	\midrule

	   8139cp &    1.32 &  122.41 &    $\times$\bf{92.58} & & 1038 &   1040 \\
	     acpi &    8.00 &   8.00  &           $\times$1.0 & &  71  &     71 \\
             e100 &   63.19 &  231.98 &     $\times$\bf{3.67} & &  573 &    569 \\
            e1000 &    3.00 &  259.06 &    $\times$\bf{86.35} & & 1427 &   1535 \\
           e1000e &    0.70 &  111.25 &   $\times$\bf{158.92} & & 1386 &   1579 \\
              gve &    2.00 &  636.22 &   $\times$\bf{318.11} & &  147 &    594 \\
         ne2k-pci & 1408.00 & 1658.00 &     $\times$\bf{1.18} & &   31 &     31 \\
             nvme &    0.02 &    0.88 &     $\times$\bf{44.0} & &  260 &    291 \\
      qemu-fw-cfg & 1254.00 &  1341.0 &     $\times$\bf{1.06} & &   35 &     37 \\
           rocker &  171.01 &  203.25 &     $\times$\bf{1.19} & &  181 &    184 \\
           sungem &    6.01 &   59.04 &     $\times$\bf{9.82} & &  924 &   1032 \\
           sunhme &  195.00 &  428.00 &     $\times$\bf{2.19} & & 1025 &   1030 \\
          tpm-tis &    2.00 &  857.00 &   $\times$\bf{428.50} & &  150 &    326 \\
      vio-balloon & 1291.00 & 1328.00 &     $\times$\bf{1.03} & &  281 &    281 \\
          vio-blk &  625.00 &  624.00 &          $\times$1.00 & &  333 &    333 \\
      vio-console &  349.00 &  444.00 &     $\times$\bf{1.27} & &  352 &    352 \\
       vio-crypto &  270.00 &  277.00 &     $\times$\bf{1.03} & &  258 &    258 \\
        vio-input &  393.00 &  635.00 &     $\times$\bf{1.62} & &  299 &    299 \\
          vio-net &  553.00 &  400.00 &          $\times$0.72 & & 1250 &   1257 \\
          vio-rng &    1.00 & 2282.00 &  $\times$\bf{2282.00} & &  238 &    239  \\
          vmxnet3 &   37.07 &   59.94 &     $\times$\bf{1.62} & &   51 &     51 \\

	\bottomrule
      \end{tabular}
    \end{threeparttable}%
  \end{center}
\label{tbl:dynamic-execs}
\end{table}


To evaluate the improvement through delay reduction, we measured the difference in path coverage and executions per second with and without the optimization. %
We ran one instance of \coolname{} for each driver listed in Table~\ref{tbl:all_bugs}.
The execution was terminated after three hours, or after $128$ restarts in cases where bugs were triggered shortly after the start of the analysis.
To improve the analysis results, we patched identified bugs when possible, as detailed in our repository~\cite{fuzzsarepo}.
For the evaluation of network drivers, we used the more elaborate harness components for network, character and block device drivers, that are provided by \coolname{}.
These components load the driver, obtain the resources created by the driver, perform a small set of system calls on the resources and unload the driver again.
Each harness contains a concurrent thread that blocks until a workload initiated by the driver enters a blocked state,
in which case the routine is woken to trigger an interrupt.
All the \gls{VIRTIO} drivers were analyzed in \textit{simulation} mode.

Table~\ref{tbl:dynamic-execs} shows the difference in execution speed between the optimized and the un-optimized version.
To account for differences in performance due to increased code coverage, we additionally list the total number of covered paths.
The table shows that reducing delays issued by driver code dramatically increases performance for most drivers without a negative impact on code coverage.
We measure an average performance improvement by a factor of $163$ through reducing delays.
However, in some cases, we see either no significant improvement or even a slight reduction in performance.
We determined two distinct causes of this behavior.
In the first case, we see that the path coverage for drivers with little or no improvement is low.
Therefore, it is likely that the driver initialization failed early before any major interaction with the device was performed.
The second case covers \gls{VIRTIO} drivers.
These drivers are specifically designed for software device back-ends and do not rely on timeouts as much as device drivers that can also interact with real hardware.
We recommend disabling delay optimization in cases where it does not increase overall performance.
\definecolor{dodgerblue4}{rgb}{0.061,0.231,0.471}
\begin{figure}
  \centering
\resizebox{\columnwidth}{!}{%
\begin{tikzpicture}
    \begin{axis}[
	ybar,
	bar shift=0.0cm,
        xlabel={Seconds},
        ylabel={Frequency},
        xmin=1.0,
	ymode=log,
	xmode=log,
        ymin=1,
	y=0.3cm,
	bar width=0.1cm,
      ]
\addplot[black, fill=dodgerblue4, fill opacity=1.0, draw=none] table [
   col sep=comma,
   y=tiq0-1-1000,
   x=Count,
]{./figures/data/irq.csv};
\addlegendentry{Random}
\addplot[black, fill=lightgray, fill opacity=0.75, draw=none] table [
   col sep=comma,
   y=tiq1-1-1000,
   x=Count,
]{./figures/data/irq.csv};
\addlegendentry{Targeted}

\end{axis}
\end{tikzpicture}}
  \caption{Distribution of the time in seconds required to trigger a bug in the \texttt{rocker} driver with targeted and random interrupt injection.}
  \label{fig:irq}
\end{figure}

We focused on the \texttt{rocker} driver to evaluate whether targeted interrupt injection improves the bug-finding capabilities of \coolname.
The \texttt{rocker} driver was selected for this evaluation
because it requires multiple interrupts to be triggered during its initialization.
If no interrupt is triggered within a fixed time window, the initialization fails.
To evaluate the effectiveness of the optimization, we ran two instances of \coolname:
one instance used targeted interrupt injection; the other injected interrupts at random time intervals ranging from $1-1000$ nanoseconds.
The experiment was repeated over $1000$ runs and each run was started with an empty corpus.
Figure~\ref{fig:irq} compares the average time in seconds required to trigger the first bug.
Overall, the optimized version took on average of $6.78$ seconds to trigger the bug, whereas the unoptimized version took $17.66$ seconds.
Targeted interrupt injection thereby reduces the time required to trigger the bug by a factor of $2.6$.

To evaluate the overall effectiveness of \coolname{} in uncovering bugs in the \gls{HV} interface of device drivers,
we measured the elapsed time until the first bug is triggered and averaged the measurement over $128$ runs.
For this evaluation, we applied the modifications to remove complex checks on data provided by the fuzzer as detailed above.
In addition, we applied patches to avoid \textit{assertion failures}, \textit{unbounded allocations} and \textit{deadlocks}.
Table~\ref{tbl:ttb} shows the results from this evaluation.
For most drivers, the first bug is triggered within the first few minutes of fuzzing,
with many bugs being triggered in under one minute of analysis.
This result demonstrates the effectiveness of \coolname{} in finding such issues,
but also underlines the extent of missing sanitization of data provided by the \gls{HV} in the Linux kernel code-base.

\begin{table}
  \caption{%
  	Time required to trigger the first Bug (TTB) in seconds for each examined driver with a known bug,
	averaged over 128 runs.
	Patches were applied to avoid low severity bugs due to assertion failures, unbounded allocations and deadlocks.
      	}
  \begin{center}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{l r | l r | l r}
      \toprule
	    %
	    & \thead{TTB (s)}
      &
	    & \thead{TTB (s)}
      &
	    & \thead{TTB (s)} \\
      \midrule
          8139cp &                         4.60 &         acpi &                     1.87 &        e100 &             1424.80 \\
	   e1000 &                        51.54 &       e1000e &                  1650.98 &         gve &              542.82 \\
	    nvme &                         0.37 &      qemu-fw &                    2.03  &      rocker &                6.78 \\
	  sungem &                         1.50 &      tpm-tis & \textsuperscript{*}7200+ & vio-balloon &               37.86 \\
	 vio-blk &                        20.24 &  vio-console &                    18.28 &  vio-crypto &               18.92 \\
	 vio-net &                         4.93 &     vio-ring &                   132.34 &     vio-rng &                2.08 \\
	 vmxnet3 &                         1.89 &              &                          &             &                     \\



      \bottomrule
    \end{tabular}}
  \end{center}
  \begin{tablenotes}
  \item \scriptsize{\textsuperscript{*} Estimate based on few runs, since the bug could not be triggered reliably.}
  \end{tablenotes}
  \label{tbl:ttb}
\end{table}



